State-of-the-art generalisation research in NLP: A taxonomy and review

The ability to generalise well is one of the primary desiderata of natural language processing (NLP). Yet, what 'good generalisation' entails and how it should be evaluated is not well understood, nor are there any evaluation standards for generalisation. In this paper, we lay the groundwork to address both of these issues. We present a taxonomy for characterising and understanding generalisation research in NLP. Our taxonomy is based on an extensive literature review of generalisation research, and contains five axes along which studies can differ: their main motivation, the type of generalisation they investigate, the type of data shift they consider, the source of this data shift, and the locus of the shift within the modelling pipeline. We use our taxonomy to classify over 400 papers that test generalisation, for a total of more than 600 individual experiments. Considering the results of this review, we present an in-depth analysis that maps out the current state of generalisation research in NLP, and we make recommendations for which areas might deserve attention in the future. Along with this paper, we release a webpage where the results of our review can be dynamically explored, and which we intend to update as new NLP generalisation studies are published. With this work, we aim to take steps towards making state-of-the-art generalisation testing the new status quo in NLP.

==> sec_discussion.tex <==
\paragraph{Efficiency}
Another type of robustness evaluation focuses less on how sensitive a model is to what specific data it is trained on, but instead on how sensitive it is to the \emph{quantity} of data it is trained on, or how often it had to see that data to converge to a solution.
It is well-known that current state-of-the-art models require very large amounts of data and compute to be trained \citep[e.g.][]{strubell-etal-2019-energy}.
It has also frequently been pointed out that humans are much more agile learners, that do not require by far as much data to learn, and that this feat should be attributed to their strong generalisation abilities \citep[e.g.][]{linzen-2020-accelerate,lake2018generalization}.
More efficient learning\footnote{
As pointed out by \citet{dehghani-etal-2021-efficiency}, there are many different ways to measure and define efficiency, which do not always correlate with each other. Here, we abstract away over that, and consider any paper that considers measures of efficiency in the context of generalisation.}
can thus be used as an indicator of good generalisation abilities.
Generalisation is evaluated from that perspective by for instance \citet{wilcox-etal-2019-structural}, who show that adding structural supervision to recurrent models helps them learn grammatical dependencies more efficiently.
\citet{yogatama2019learning}, instead, consider efficiency as a metric to quantify generalisation even more explicitly and argue that a model that requires 100 examples to achieve 90\% accuracy should be preferred over a model that requires 10$^6$ examples to get to 92\% accuracy.
In their metric of efficiency, interestingly, they also take into account compressibility, another concept related to generalisation \citep[e.g.][]{wolff1982language}.
Interestingly, while the field generally agrees on the importance of (sample) efficiency, from a responsibile as well as a practical perspective, most recent work instead focuses on what changes in models when \emph{more} data is presented to them \citep[e.g.][]{bahri-etal-2021-explaining,kaplan-etal-2020-scaling,gordon-etal-2021-data}.






==> subsec_types_of_generalisation.tex <==
\subsection{Types of generalisation}

As already pointed out in the introduction, the standard setting for measuring generalisation of ML models is to randomly split the data into three or more sets, and use one of those for model evaluation. 
It is worth pointing out that even in this most basic setup, test set scores reflect generalisation.
After all, the test data is different from the training (and validation) data.
In the past decennium, neural models have made large leaps when it comes to this kind of random-split generalisation which, following the distributional similarities between train and test data, is often called \emph{within-distribution generalisation}.
With this impressive progress, however, also came the realisation that high or human-ceiling scores on test sets drawn from the same distribution as the training data do not necessarily imply that models are in fact strong-generalisers.
A range of recent studies has exposed a manifold of \emph{generalisation failures} in models that achieve super-human performance when tested on within-distribution generalisation \citep[i.a.]{linzen-2020-accelerate,lake2017building,lake2018generalization,kaushik2019learning,gardner-etal-2020-evaluating}.
Such studies consider a different type of generalisation, called \emph{out-of-distribution} generalisation, where the test data distributionally differs from what the model has seen during training, for instance because new words or combinations of words are introduced \citep{lake2018generalization} or the input data comes from a different demographic of the population \citep{plank2016non}.

In the broader field of machine learning, it is common to describe out-of-distribution generalisation by the way in which thee training data differs from the evaluation data.
This more finegrained categorisation contains three different types of `shifts': \emph{covariate shift}, where the distributional difference occurs in the input features ($p_{\text{test}}(x) \not= p_{\text{train}}(x)$), \emph{label shift}, where instead there is a change in labels ($p_{\text{test}}(y) \not= p_{\text{train}}(y)$), and  concept shift, where there is a shift in the conditional distribution of the labels given the input ($p_{\text{test}}(y|x) \not= p_{\text{train}}(y|x)$).
% 
Most examples of generalisation evaluation in NLP are examples of \emph{covariate shift}, characterised by a mismatch in the distribution of input features.
For instance, the earlier mentioned work of \cite{mccoy-etal-2019-right}, exposes failures of state-of-the-art NLI models by constructing input examples with slightly different input features, such that heuristics such as lexical or constituent overlap are not sufficient anymore for solving the task. %TODO rewrite
% For instance, in \citeauthor{mccoy-etal-2019-right}'s NLI test, the inputs are constructed such that the relevant predictive features remain the same, but particular heuristical input properties that are predictive for the training examples (e.g.\ word overlap between premise and hypothesis) are not.
Label and concept shift are less common in NLP generalisation research, although shifts in the input data distribution can also results in shifts in the distribution of the output labels and their conditional probabilities.
When there are shifts in genre or topic, as in the cases described by \citet{plank2016non}, identical words or phrases might be used differently (concept shift), or have a different interpretation (label shift).
Consider, for example, the meaning of the phrase \emph{it doesn't run}, which has a vastly different meaning (concept shift) as well as sentiment (label shift) in a review for software and a review for mascara.
 
However, although generalisation in NLP and linguistics could be cast into these more general and formal notions of in- and out-of-distribution, in practice, these are not the dimensions along which generalisation is usually considered.
Instead, researchers in the field consider aspects such as sample-efficiency \citep{linzen-2020-accelerate,yogatama2019learning}, adaptation to different domains \citep{plank2016non}, whether models can generalise \emph{compositionally} \citep[e.g.][]{lake2017building,schmidhuber1990towards,wong2007generalisation} -- often contrasted with memorising the training data \citep[e.g.][]{elangovan-etal-2021-memorization,korrel-etal-2019-transcoding} -- and to what extent they generalise across different tasks or languages \citep[e.g.][]{yogatama2019learning,hu2020xtreme}.
In the rest of this section, we discuss five popular approaches, as well as their main conclusions.

